What can Large Language Models do in chemistry? A comprehensive benchmark on eight tasks

Large Language Models (LLMs) with strong abilities in natural language processing tasks have emerged and have been applied in various kinds of areas such as science, finance and software engineering. However, the capability of LLMs to advance the field of chemistry remains unclear. In this paper, rather than pursuing state-of-the-art performance, we aim to evaluate capabilities of LLMs in a wide range of tasks across the chemistry domain. We identify three key chemistry-related capabilities including understanding, reasoning and explaining to explore in LLMs and establish a benchmark containing eight chemistry tasks. Our analysis draws on widely recognized datasets facilitating a broad exploration of the capacities of LLMs within the context of practical chemistry. Five LLMs (GPT-4, GPT-3.5, Davinci-003, Llama and Galactica) are evaluated for each chemistry task in zero-shot and few-shot in-context learning settings with carefully selected demonstration examples and specially crafted prompts. Our investigation found that GPT-4 outperformed other models and LLMs exhibit different competitive levels in eight chemistry tasks. In addition to the key findings from the comprehensive benchmark analysis, our work provides insights into the limitation of current LLMs and the impact of in-context learning settings on LLMs' performance across various chemistry tasks. The code and datasets used in this study are available at https://github.com/ChemFoundationModels/ChemLLMBench.

==> 1-introduction.tex <==
\section{Introduction}
% Why is it so urgent and attractive to do this evaluation? 
% 1. llm performs well Complex Reasoning in other tasks; 
% 2. For the science area, there are some works, in medical..., but only a few works for chemistry, and these works are not comprehensive and lack insights into LLM. 
% 3. LLMs may revolutionize the chemistry field
% 4. So it's urgent and attractive and we do this evaluation
Large language models (LLMs)  have recently demonstrated impressive  reasoning abilities across a wide array of tasks.
These tasks are not limited to natural language processing, but also extend to various language-related applications within scientific domains~\cite{taylor2022galactica, gptmedical, hendrycks2021ethics, hendryckstest2021}. Much of the research on the capacity of LLMs in science has been focused on tasks like answering of medical ~\cite{gptmedical} and scientific questions ~\cite{hendrycks2021ethics, hendryckstest2021}. However, the exploration of their application to practical tasks in the field of chemistry remains underinvestigated.
%such as recommending systems~\cite{gptrecommend}, science~\cite{galactica, gptmedical, hendrycks2021ethics, hendryckstest2021}.
%, finance~\cite{bloomberggpt}.
%there have been previous investigations into the capabilities of large language models in some domains and tasks. However, most of them focus  on medical question answering~\cite{gptmedical}, scientific question answering~\cite{hendrycks2021ethics, hendryckstest2021}. However, there has been limited research on the application of these models to chemistry practical tasks. 
Although some studies~\cite{castro2023large,jablonka2023gpt, adllmcode, ramos2023bayesian} have been conducted, they tend to focus on a specific case studies rather than a comprehensive or systematic evaluation. The exploration of LLMs' capabilities within the field of chemistry has the potential to revolutionize this domain and expedite research and development activities.  Thus, the question, \textbf{\textit{``What can LLMs like GPT models do in chemistry?''}}  is a compelling topic of inquiry for both AI researchers and chemists. In order to address this knowledge gap, we have developed a comprehensive benchmark to provide a preliminary investigation into the abilities of GPT models across a diverse range of practical chemistry tasks. Our aim is to gain insights that
 will be beneficial for both AI researchers and chemists in order to advance the application of GPT models in chemistry.
% Who cares and will benefit from this paper
% 1. Chemist: Many tasks, All in one, unified 
% 2. AI researcher: Different Prompt, In-context learning, Samples
%Our benchmark and investigation seeks to explore the potential abilities of LLMs in chemistry, offering several benefits for both AI researchers and chemists. 
For AI researchers, we provide insights into the strengths, weaknesses, and limitations of LLMs in chemistry-related tasks, which can inform further development and refinement of different AI techniques for more effective applications within the field. For chemists, our study provides a better understanding of the extent to which they can rely on current GPT models.  Utilizing our more extensive experimental setup, a broader range of chemistry tasks can be explored to further evaluate the capabilities of LLMs. %Based on our systematic experiment setup, more chemistry tasks can be conducted to investigate the abilities of LLMs in them.


% Our Key findings
% 1. Worse   Classification: competitive   Generative: Reaction/Retro
% 2. Model: gpt4 >= davinci003 > gpt3.5
% 3. Method: ICL > Zero-shot; How to find icl examples; number of ICL examples => quality and quantity

{Our investigation focus on 8 practical chemistry tasks,   which cover a wide spectrum of the chemistry domain. These include:}  1) name prediction, 2) property prediction, 3) yield prediction, 4)  reaction prediction, 5) retrosynthesis (prediction of reactants from products),  6) text-based molecule design, 7) molecule captioning, and 8) reagents selection. Our analysis draws on widely available datasets including BBBP, Tox21~\cite{wu2018moleculenet}, PubChem~\cite{kim2019pubchem}, USPTO~\cite{jin2017predicting, schneider2016s}, ChEBI~\cite{edwards2022translation, edwards-etal-2021-text2mol}, and so on.
Three GPT models (GPT-4, GPT-3.5, and Davinci-003)~\cite{openai2023gpt4} are evaluated for each chemistry task in  zero-shot and few-shot in-context learning settings with carefully selected demonstration examples and specific prompts.

The \textbf{main findings} from the investigations are: \vspace{-0.1in}
\begin{itemize}
    \item GPT-4 outperforms the other two models among the three evaluated. The ranking of the three models on 8 tasks can be found in Table \ref{rank}; 
    \item GPT models exhibit less competitive performance in tasks demanding precise understanding of molecular SMILES representation, such as name prediction, reaction prediction and retrosynthesis; 
    \item GPT models demonstrate strong capabilities in text-related explanation tasks such as molecule captioning; \item For chemical problems that can be converted to classification tasks or ranking tasks, such as property prediction, and  yield prediction, GPT models can achieve competitive performance compared to baselines that use classical machine learning (ML) models as classifiers, or even better,  as summarized in   Table \ref{rank}. \vspace{-0.1in}
\end{itemize}
These conclusions are derived from conducting five repeated evaluations on each task, using the best evaluation setting that was discovered through a grid search on the validation set of each task.

Based on our analysis, specifically from formulating prompts and preparing demonstration examples for in-context learning, we have derived the following \textbf{recommendations} for AI researchers and chemists who are considering using LLMs for future chemistry tasks: \vspace{-0.1in}
\begin{itemize}
    \item In-context learning (ICL) achieves a  significantly better performance than zero-shot prompting. It is thus crucial to  develop methods for identifying in-context learning examples that have the potential to greatly enhance performance;
    \item ICL examples identified by similarity-based search are more useful than randomly sampled ones;
    \item Having a greater number of ICL examples is preferable over a limited number. 
\end{itemize} \vspace{-0.1in}
These suggestions are derived from analyzing the results of 12 different variants of each option and evaluating their performance on the validation set.
%1. Through extensive experiments, we find that GPT models perform well in explaining tasks but poorly in generative tasks specifically evaluated by the exact match (accuracy) metric such as reaction prediction, and retrosynthesis. For chemical problems that can be converted to classification tasks or ranking tasks such as property prediction, and reaction yield prediction, GPT models can achieve competitive performance compared to baselines. 2. As shown in Table \ref{rank}, GPT-4 is a little better than Davinci-003 and both are better than GPT-3.5 across most tasks. 3. In terms of the prompting methods, in-context learning (ICL) achieves a more significant performance than zero-shot prompting. It's very necessary and important to design ways to find in-context learning examples because high-quality examples can boost performance. Additionally, a greater quantity of ICL examples is preferable to a limited number.


% Extensive experiments and conclusions
% 1. Benchmark
% 2. Experiment setup
% 3. Results and insights
We highlight the \textbf{contributions} of this paper as follows: \vspace{-0.1in}
\begin{itemize}
  \item We are the first to establish a comprehensive benchmark to evaluate the abilities of LLMs on a wide range of chemistry tasks. These eight selected tasks, in consultation with chemists, not only encompass a broad spectrum of the chemistry domain but also demand various abilities such as comprehension, reasoning, and explanation using domain-specific chemistry knowledge. The selected tasks and datasets thus provide a comprehensive and representative overview for benchmarking purposes.
  \item We provide a comprehensive experimental framework for testing of LLMs in chemistry tasks. To factor in the impact of prompts and demonstration examples in zero-shot and in-context learning, we have assessed multiple input options for the GPT models, focusing on the description of chemistry tasks. Five representative  configurations were chosen based on their performance on a validation set, then these selected options were applied on the testing set. The conclusion is made from five repeated evaluations on each task since GPTs often yield different outputs at different API calls even though the input is the same. We thus believe that our benchmarking process is both reliable and systematic.   %To make the evaluation trustable and systematical, we identified key evaluation problems, models, and factors that may influence the performance and conduct extensive experiments (zero-shot and in-context learning).
  \item Our investigations yield broader insights into the performance of GPT models on chemistry tasks. While confirming some anticipated outcomes, they also offer unexpected findings. Our work also led to practical recommendations that can guide AI researchers and chemists in leveraging GPT models more effectively in the future.  We believe that  
  %that Large Language Models (LLMs) underperform in comparison to baseline models when evaluated on partial datasets with an in-context learning setting. However, this outcome hints at the intriguing potential of LLMs. Particularly, 
  this preliminary investigation offers crucial perspectives for AI researchers and chemists alike, deepening our comprehension  of LLMs' capacities and fostering additional research at the intersection of LLMs and chemistry.
\end{itemize}



% Table for the rank of different LLMs
\begin{table}[!h]
%\begin{wraptable}[11]{r}{0.5\textwidth}
\centering \vspace{-0.02in}
\caption{The rank of three GPT models on eight chemistry tasks and performance highlight (NC: not competitive, C: competitive, SC: selectively competitive, acc: accuracy). }
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|c|c|c|l}
\toprule
Task                      & \multicolumn{1}{l|}{GPT-4} & \multicolumn{1}{l|}{GPT-3.5} & \multicolumn{1}{l|}{Davinci-003} & Performance highlight (comparing to  baselines if any) \\ \midrule
\hyperref[sec:np]{Name Prediction}            & 1                          & 2                            & 3                         & \textbf{NC}: max. acc. 8\%   (Table \ref{name_prediction_results})  \\ \midrule
\hyperref[sec:pp]{Property Prediction}      & 1                           &           2                   &   3          & \textbf{SC}: outperform  MoIR \cite{wang2021chemical} (Table \ref{pp_f1_table})                     \\ \midrule
\hyperref[sec:yp]{Yield Prediction}  & 1                           & 3                             &  2                &  \textbf{C}: but 16-20\% lower acc. than UAGNN \cite{kwon2022uncertainty}     (Table \ref{tab:yld-table})     \\ \midrule
\hyperref[sec:rp]{Reaction Prediction}      & 1                          & 3                            & 2                &     \textbf{NC}: 70\% lower  acc.  than Chemformer~\cite{irwin2022chemformer}    (Table \ref{reaction_prediction_results})      \\ \midrule
\hyperref[sec:rs]{Reagents Selection}         & 2                          &1                            & 3                          &    \textbf{C}: 40-50\% acc. (Table \ref{reagents_table})  \\ \midrule
\hyperref[sec:retro]{Retrosynthesis}            & 2                          & 3                            & 1                            &  \textbf{NC}: 40\% lower  acc. than Chemformer~\cite{irwin2022chemformer}    (Table \ref{retro_results}) \\ \midrule
\hyperref[sec:text_basedmd]{Text-Based Molecule Design}           & 1                          & 3                            & 2          &       \textbf{SC}:    better than   MolT5-Large~\cite{edwards2022translation}   (Table \ref{text_based_moldesign_results})       \\ \midrule
\hyperref[sec:mc]{Molecule Captioning}       & 1                          & 2                            & 1                   &    \textbf{SC}:   better than   MolT5-Large~\cite{edwards2022translation}   (Table \ref{captioning_results})       \\ \midrule
Average   rank              &    1.25                    &           2.375                      &                2.125        & overall:  3 \textbf{SC},  2 \textbf{C},   3 \textbf{NC}   \\ \bottomrule
\end{tabular}}
\label{rank}
\end{table}
%\end{wraptable}

The paper is organized as follows: In section \ref{sec:method}, we elaborate on the evaluation process, including an overview of the chemistry tasks, the utilized GPT models and prompts, and the validation and testing settings. Then we provide details of the evaluation on each  chemistry task, in the following order: 
name prediction in section \ref{sec:np}, property prediction in section \ref{sec:pp},
 yield prediction in section \ref{sec:yp},  
reaction  prediction in section \ref{sec:rp},
reagents selection in section \ref{sec:rs}, 
retrosynthesis (prediction of reactants from products) in section \ref{sec:retro},
text-based molecule design in section \ref{sec:text_basedmd}, and molecule captioning in section \ref{sec:mc}. Finally,   to answer the question \emph{What indeed can GPT models do in chemistry?} we share our findings and discuss the constraints inherent to LLMs  and how different settings related to LLMs affect performance across various chemistry tasks in section \ref{sec:discussion}. Related works  are presented in  section \ref{sec:related-work}, and the conclusions are summarized in section \ref{sec:conclusion}.

% Why you can Trust us?
% 1. How many Tasks 9; How many Dataset; Test size distribution 
% 2. davinci-003, 3.5, GPT-4 
% 3. Experiment process: valid-30, test-100, randomly, repeat 5 times mean and variance 
% 4. Baselines
%To make this evaluation trustable, comprehensive, and rigorous, we list some key questions for a better evaluation: 
%\begin{itemize}
 %   \item What kinds of tasks and datasets need to be used to evaluate the abilities of LLMs?
%    \item There are many different kinds of LLMs and different factors which can influence the prompting result. How to evaluate them?
%    \item How to reduce the influence of the LLMs randomness on the results?
%\end{itemize}
%To solve these questions, we first identify 3 key abilities including understanding, reasoning, and explaining to investigate and then we construct 8 widely researched chemistry tasks including molecule property prediction, reaction prediction, molecule design, etc. We collected commonly employed datasets like USPTO, ChEBI, HIV, etc., and identified the evaluation metrics accordingly. We then conduct an evaluation of the leading Language Learning Models (LLMs) such as GPT-4, Davinci-003, and GPT-3.5. Through our extensive experiments, we identify two key factors: the similarity search methods and the number of in-context learning samples which will influence the in-context learning. Considering the combinations of the LLMs, and in-context learning factors (temperature, In-context learning example size,etc), we conduct 12 different variants of these choices. To save the consumption of API requesting, for each task, we first construct a validation set of size 30 and test these different choices on the validation set. Then based on the results, we choose 5 representative choices and apply them to a test set of size 100 randomly sampled from the original dataset. To reduce the influence of the LLMs randomness on the results, each experiment is repeated for 5 times and the mean and variance are reported. We also select baseline for comparison for each task.

==> 100-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
